CoughTrigger: Earbuds IMU Based Cough Detection Activator Using An Energy-efficient Sensitivity-prioritized Time Series Classifier

Persistent coughs are a major symptom of respiratory-related diseases. Increasing research attention has been paid to detecting coughs using wearables, especially during the COVID-19 pandemic. Among all types of sensors utilized, microphone is most widely used to detect coughs. However, the intense power consumption needed to process audio signals hinders continuous audio-based cough detection on battery-limited commercial wearable products, such as earbuds. We present CoughTrigger, which utilizes a lower-power sensor, an inertial measurement unit (IMU), in earbuds as a cough detection activator to trigger a higher-power sensor for audio processing and classification. It is able to run all-the-time as a standby service with minimal battery consumption and trigger the audio-based cough detection when a candidate cough is detected from IMU. Besides, the use of IMU brings the benefit of improved specificity of cough detection. Experiments are conducted on 45 subjects and our IMU-based model achieved 0.77 AUC score under leave one subject out evaluation. We also validated its effectiveness on free-living data and through on-device implementation.

==> dump_5-1_synth_result.tex <==

\subsection{Synthetic Dataset}

% To validate the usability of the self-tuning classifier. 
We created a synthetic “snowman” dataset by combining two Gaussian distributions ($\mu_1$=$(0,0)$, $\sigma_1$=$3$; $\mu_2$=$(0,3)$, $\sigma_2$=$1$) as shown in Fig.~\ref{fig:snowman} to validate our algorithm. 
The dataset has the size of 1334 samples, each of which has two non-time series features. The positive to negative ratio is about 2:1. 
We randomly select 70\% of the samples as training set and the left as test set. 
We employed this dataset to make a sanity test and compare the inference speed and model size of MCC with a large range of popular classifiers\footnote{All implemented in Python 3.7. Hardware platform: Intel i7-7500U 2.70GHz, 2 cores, 16GB RAM.}. 
Euclidean distance is used here in MCC algorithm.
Note that the comparison of inference time is actually not fair for MCC, since MCC implementation code has not been optimized for speed, in contrast to other highly-optimized algorithm implementations from a popular library (scikit-learn~\cite{sklearn} uses Cython and C functions for speedup). % It is important to know MCC is supposed to provide much faster inference speed when necessary engineering effort is paid to speed optimization. 

\begin{figure}
\centering
\hspace{-.5cm}\includegraphics[width=.3\textwidth]{figure/Screen Shot 2021-05-04 at 2.02.05 AM.png}
\caption{Synthetic snowman dataset.}
\label{fig:snowman}
\end{figure}


We compared MCC with ten popular traditional classifiers including KNN (K=1), KNN (K=3), Linear SVM, Radial Basis Function (RBF) SVM, Decision Tree (DT), Random Forest (RF), Quadratic Discriminant Analysis (QDA), AdaBoost, Naive Bayes, and Neural Network (NN) with 1 hidden layer and 100 neurons. All the baselines are imported from scikit-learn library~\cite{sklearn}. We saved each trained model locally after training. For MCC, we saved both the classifier itself and the obtained centroids with thresholds. 

When implementing MCC, the cost threshold can be replaced by accuracy threshold, which allows direct manipulation of desired test accuracy (if the training set and test set have identical distribution). 
It is such an advanced and practically useful feature that we can adjust the accuracy threshold to balance the accuracy and inference time.
% 
We tested MCC classifier with two different accuracy thresholds: MCC (T1) with 0.9 threshold and MCC (T2) with 0.95 threshold. 
MCC (T1) classifier gained 90.1\% training accuracy with two centroids converged, and test accuracy of 95.9\%. MCC (T2) has 96.9\% training accuracy with 14 centroids, and the test accuracy is 99.2\%.
% 

After repeating each method for 1000 times, we show the averaged inference time V.S. accuracy in Fig.~\ref{fig:speed}. 
\change{MCC (T1) has an inference time of 0.062 ms and MCC (T2) takes 0.42 ms on average. Both of our MCC classifiers have shorter inference time than any of the baseline methods. In terms of test accuracy, MCC (T2) has achieved the best score (99.2\%), even better than KNN (K=1) due to its superior robustness, i.e., resistance to noise.} 
% 
We then present the accuracy V.S. model size in Fig.~\ref{fig:model size}. It can be observed that our classifier provides a superior performance in aspect of model size, which is of important significance to low-resource embedded systems. It's worth noticing that our model can also be further optimized to be more space-efficient. %, as well as the data type stored on chip.

% TODO:\textcolor{red}{how many centers found}




% https://scikit-learn.org/stable/
% https://tslearn.readthedocs.io/en/stable/



\begin{figure}
\centering
\vspace{.1cm}\includegraphics[width=.497\textwidth]{figure/speed.jpg}
\caption{Comparison of the accuracy V.S. inference time of different models on synthetic dataset.}
\label{fig:speed}
\end{figure}
%  (\change{Note that our MCC implementation could be further optimized for speed,} in contrast to other algorithms imported from scikit-learn.)


\begin{figure}
\centering
\includegraphics[width=.48\textwidth]{figure/mdl_size.jpg}
\caption{Comparison of accuracy V.S. model size of different models on synthetic dataset.}
\label{fig:model size}
\end{figure}


% @misc{UCRArchive,
% title={The UCR Time Series Classification Archive},
% author={ Chen, Yanping and Keogh, Eamonn and Hu, Bing and Begum, Nurjahan and Bagnall, Anthony and Mueen, Abdullah and Batista, Gustavo},
% year={2015},
% month={July},
% note = {\url{www.cs.ucr.edu/~eamonn/time_series_data/}}
% }


% \subsection{UCI Benchmark Corpus}


\subsection{UCR Trace Dataset}

% \textcolor{red}{[INTRODUCE TRACE]}

We used UCR Trace dataset~\cite{UCRArchive} to test its usability and inference speed in times series classification problems. The dataset size is 200, and the time series length is 275. There are 4 classes in the original dataset. We combined class 2 and 3 as training set and class 1 and 4 as test set. The positive and negative ratio is 1:1. We made a 7/3 ratio train/test set random split.
% 
Since it is acknowledged that 1NN-DTW provides very accurate performance for time series classification problems, we use 1NN-DTW (implementation from tslearn library~\cite{tslearn}) as our baseline. The test accuracy is 100\%, and inference time is 2.1 s. The saved model size is 45 KB.
% 
Our MCC finished at 2 clusters discovered and also a 100\% accuracy is achieved. The inference time is 0.011 s, which is 190 times shorter than baseline.
% 
The model size is 1 KB, which is 45 times smaller than baseline, when we save both the templates (with threshold) and the model. 

